Efficient Traffic Prediction Through Spatio-Temporal Distillation

Graph neural networks (GNNs) have gained considerable attention in recent years for traffic flow prediction due to their ability to learn spatio-temporal pattern representations through a graph-based message-passing framework. Although GNNs have shown great promise in handling traffic datasets, their deployment in real-life applications has been hindered by scalability constraints arising from high-order message passing. Additionally, the over-smoothing problem of GNNs may lead to indistinguishable region representations as the number of layers increases, resulting in performance degradation. To address these challenges, we propose a new knowledge distillation paradigm termed LightST that transfers spatial and temporal knowledge from a high-capacity teacher to a lightweight student. Specifically, we introduce a spatio-temporal knowledge distillation framework that helps student MLPs capture graph-structured global spatio-temporal patterns while alleviating the over-smoothing effect with adaptive knowledge distillation. Extensive experiments verify that LightST significantly speeds up traffic flow predictions by 5X to 40X compared to state-of-the-art spatio-temporal GNNs, all while maintaining superior accuracy.

==> check.tex <==
\section{Reproducibility Checklist}
% Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced [{\color{blue}{Yes}}]
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results [{\color{blue}{Yes}}]
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper [{\color{blue}{Yes}}]
    \item Does this paper make theoretical contributions? [{\color{blue}{Yes}}]
\end{itemize}

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. [{\color{blue}{Yes}}]
\item All novel claims are stated formally (e.g., in theorem statements). [{\color{blue}{Yes}}]
\item Proofs of all novel claims are included. [{\color{blue}{Yes}}]
\item Proof sketches or intuitions are given for complex and/or novel results. [{\color{blue}{Yes}}]
\item Appropriate citations to theoretical tools used are given. [{\color{blue}{Yes}}]
\item All theoretical claims are demonstrated empirically to hold. [{\color{blue}{Yes}}]
\item All experimental code used to eliminate or disprove claims is included. ([{\color{blue}{Yes}}]
\item Does this paper rely on one or more datasets? [{\color{blue}{Yes}}]
\end{itemize}

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets [{\color{blue}{Yes}}]
    \item All novel datasets introduced in this paper are included in a data appendix. [{\color{blue}{NA}}]
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. [{\color{blue}{NA}}]
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. [{\color{blue}{Yes}}]
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. [{\color{blue}{Yes}}]
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing.  [{\color{blue}{Yes}}]
    \item Does this paper include computational experiments?  [{\color{blue}{Yes}}]
\end{itemize}
If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix.  [{\color{blue}{Yes}}]
\item All source code required for conducting and analyzing the experiments is included in a code appendix.  [{\color{blue}{Yes}}]
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.  [{\color{blue}{Yes}}]
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from  [{\color{blue}{Yes}}]
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results.  [{\color{blue}{Yes}}]
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks.  [{\color{blue}{Yes}}]
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. [{\color{blue}{Yes}}]
\item This paper states the number of algorithm runs used to compute each reported result.  [{\color{blue}{Yes}}]
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. [{\color{blue}{NA}}]
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank).  [{\color{blue}{Yes}}]
\item This paper lists all final hyperparameters used for each model/algorithm in the paper's experiments.  [{\color{blue}{Yes}}]
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting.  [{\color{blue}{Yes}}]
\end{itemize}

